Leveraging Vision Reconstruction Pipelines for Satellite Imagery

Reconstructing 3D geometry from satellite imagery is an important topic of research. However, disparities exist between how this 3D reconstruction problem is handled in the remote sensing context and how multi-view reconstruction pipelines have been developed in the computer vision community. In this paper, we explore whether state-of-the-art reconstruction pipelines from the vision community can be applied to the satellite imagery. Along the way, we address several challenges adapting vision-based structure from motion and multi-view stereo methods. We show that vision pipelines can offer competitive speed and accuracy in the satellite context.

==> 07-future_work.tex <==
\section{Future Work}
In this work, we demonstrated the feasibility of leveraging vision reconstruction pipelines to tackle reconstruction from satellite images. Possible future research directions would include unleashing our plane sweep stereo with more views. 
